Fighting Fire with Fire: Avoiding DNN Shortcuts through Priming

Across applications spanning supervised classification and sequential control, deep learning has been reported to find "shortcut" solutions that fail catastrophically under minor changes in the data distribution. In this paper, we show empirically that DNNs can be coaxed to avoid poor shortcuts by providing an additional "priming" feature computed from key input features, usually a coarse output estimate. Priming relies on approximate domain knowledge of these task-relevant key input features, which is often easy to obtain in practical settings. For example, one might prioritize recent frames over past frames in a video input for visual imitation learning, or salient foreground over background pixels for image classification. On NICO image classification, MuJoCo continuous control, and CARLA autonomous driving, our priming strategy works significantly better than several popular state-of-the-art approaches for feature selection and data augmentation. We connect these empirical findings to recent theoretical results on DNN optimization, and argue theoretically that priming distracts the optimizer away from poor shortcuts by creating better, simpler shortcuts.

==> 3_theory.tex <==
We now state our theoretical results as follows, starting from the basic definitions and assumptions.

\textbf{Data Distribution.}
Let $(\x, \y) \sim \cP_{in} \subset \bR^d \times \bR$, $(\z, \y) \sim \cP_{out} \subset \bR^d \times \bR$ denote the input and the corresponding label in the \emph{training region} and \emph{test region}, respectively.
Without loss of generality, we assume that $\bE \x =  \bE \z = \boldsymbol{0}$, and $ |\y| \leq O(1)$ is bounded almost surely.
For simplicity, we assume the data covariance satisfies $\Sigma = \Sigma_{\x} = \Sigma_{\z}$, and assume that $\operatorname{Tr}(\Sigma) = d$, $\sigma_{min} (\Sigma) = O(1)$, and $\sigma_{max} (\Sigma) = O(1)$.
We assume that the re-scaled input $\Sigma^{-1/2} \x$ and $\Sigma^{-1/2} \z$ has independent and $O(1)$-subGaussian coordinates.

Denote the optimal linear estimator as $\beta^*$, which satisfies $\bE_{\cP_{in}}(\y - \x^\top \beta^*) = \min_\beta \bE_{\cP_{in}}(\y - \x^\top \beta)$, and $\|\beta^* \| = O(1)$.
We assume that the residual $\boldsymbol{\epsilon} = \y - \x^\top \beta^*$ is mean zero, independent, $O(1)$-subgaussian conditional on $\x$ with $\bE \boldsymbol{\epsilon}^2|\x = O(1) $.
Given the dataset with $n$ pairs independently sampled from $\cP_{in}$ and $\cP_{out}$, we denote the empirical distribution by $\hat{\cP}_1^n$ and $\hat{\cP}_2^n$.
We assume that the sample size satisfies $n \gg d$ and $n = d^{O(1)}$, and the corresponding design matrix is diagonalizable.

\textbf{Model.}
We consider a two-layer fully-connected neural network with $m$ hidden neurons: $f(\x; \w, v):=\frac{1}{\sqrt{m}} \sum_{r=1}^m v_r \sigma(\w_r^\top\x/\sqrt{d})$ with symmetric initialization, where the activation $\sigma$ is smooth or piece-wise linear.
In this paper, \emph{Neural Tangent Kernels (NTK)} are applied to approximate the neural networks\footnote{The neural tangent kernel regime is widely considered in theoretical analysis as a surrogate to neural networks, since neural networks converge to the neuron tangent kernel as its width goes to infinity.}, where $\{ \w_r \}$ is trainable and $\{v_r\}$ is fixed following the regime in \citet{DBLP:conf/icml/AroraDHLW19}.
For the training process with constant step size (sufficiently small) and $\ell_2$ loss, we derive the following Theorem~\ref{thm: mainTheorem} for the function $f_{NTK}(\cdot)$ trained at time $t$

\begin{theorem}
\label{thm: mainTheorem}
Let $\alpha \in (0, 1/4)$ be a fixed constant. 
Let $h(\x) = \x^\top \beta^*: \bR^d \to \bR$ denote a linear model, and $g: \bR^d \to \bR$ denote another model.
We assume the following (A1-A3) assumptions\footnote{
We denote $ \| x_1 - x_2 \|_{\mu} = (\bE_{\mu} (x_1 - x_2)^2 )^{1/2}$}:
\begin{enumerate}
    \item[A1] In the training region $\cP_{in}$, function $f$ and $g$ are both close to the ground truth, 
    $\| y -  h(\x) \|_{\cP_{in}} \leq \epsilon$, and $\| y -  g(\x) \|_{\cP_{in}} \leq \epsilon$.
    \item[A2] In the test region $\cP_{out}$, function $f$ and $g$ are separable,  $\| g(\x) -  h(\x) \|_{\cP_{out}}\geq O(1)$.
    \item[A3] The width of the neural network satisfies $m =\Omega(  d^{1+\alpha} )$ 
\end{enumerate}
Then for the model $f_{NTK}^{t}(\cdot)$ trained by neural tangent kernel at time $t = \Theta(d^{1+\frac{1}{3}\alpha})$, satisfies the following statements (C1-C2) hold with high probability\footnote{The probability is taken over the random initialization, the training samples, and the test samples}:
\begin{enumerate}
    \item[C1] In training region $\cP_{in}$, the trained model reaches small training error, $\| f_{NTK}(\x) - y \|_{\hat{\cP}_1^n} - \epsilon \lesssim d^{-\frac{1}{3} \alpha} + \sqrt{\frac{d}{n}}$.
    \item[C2] In test region $\cP_{out}$, the trained model is closer to $f$ instead of $g$, $\| f_{NTK}(\x) - h \|_{\hat{\cP}_2^n} \lesssim d^{-\frac{1}{3} \alpha} + \sqrt{\frac{d}{n}}$ and $\| f_{NTK}(\x) - g \|_{\hat{\cP}_2^n} = \Omega(1)$. 
\end{enumerate}
\end{theorem}

Theorem~\ref{thm: mainTheorem} validates that neural networks (approximated by neural tangent kernels) indeed have different preferences in terms of different types of input. 
In the training region, function $h$ (which is linear in the input features) and function $g$ approximate the ground truth $\y$ (Assumption~A1). 
Therefore, the trained classifier can learn the pattern of $h$ or $g$ to reach a small training error.
However, $h$ and $g$ perform pretty differently on the test region (Assumption~A2).
Theorem~\ref{thm: mainTheorem} demonstrates that neural networks indeed prefer the simple function $h$, which is linear in the input features.
Taking advantage of this property, We can manipulate the model preference by providing different input features.


